Low Power Wide Area Networks: An Overview

Low Power Wide Area (LPWA) networks are attracting a lot of attention primarily because of their ability to offer affordable connectivity to the low-power devices distributed over very large geographical areas. In realizing the vision of the Internet of Things (IoT), LPWA technologies complement and sometimes supersede the conventional cellular and short range wireless technologies in performance for various emerging smart city and machine-to-machine (M2M) applications. This review paper presents the design goals and the techniques, which different LPWA technologies exploit to offer wide-area coverage to low-power devices at the expense of low data rates. We survey several emerging LPWA technologies and the standardization activities carried out by different standards development organizations (e.g., IEEE, IETF, 3GPP, ETSI) as well as the industrial consortia built around individual LPWA technologies (e.g., LORa Alliance,WEIGHTLESS-SIG, and DASH7 Alliance). We further note that LPWA technologies adopt similar approaches, thus sharing similar limitations and challenges. This paper expands on these research challenges and identifies potential directions to address them. While the proprietary LPWA technologies are already hitting the market with large nationwide roll-outs, this paper encourages an active engagement of the research community in solving problems that will shape the connectivity of tens of billions of devices in the next decade.

==> chronosyschr.tex <==
% This is is the main file of the `chronosys' package, with all the principal code.
%
% The maintener of this work is Mathieu Long.
% email : mlong.tex@hotmail.fr
% the `chronosys' package consists in the 9 files :
%  -- `docchronosys_en.tex' and `docchronosys_en.pdf' (english manual)
%  -- `docchronosys_fr.tex' and `docchronosys_fr.pdf' (french manual)
%  -- README
%  -- `chronosys.tex' (file for plain TeX)
%  -- `chronosyschr.tex' (main file of the `chronosys' package)
%  -- `chronosys.sty' (file for LaTeX)
%  -- `x-chronosys.tex' (file for ConTeXt)
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is Mathieu Long.
%
\expandafter\ifx\csname chronosys @\endcsname\relax\else\immediate\write16{Le fichier a deja ete charge}\endinput\fi
\ifx\numexpr\UNDEFINED\immediate\write16{Desole, mais ce fichier utilise les primitives E-TeX, vous ne pouvez pas utiliser le moteur TeX.}\endinput\fi
\expandafter\edef\csname chronosys @\endcsname{\the\catcode`\@}%
\catcode`\@=11%
\catcode`\!=11%
\def\chron@sysversion{1.2}%
%
\newhelp\chrhelpmessage{Contactez l'auteur par mail.}%
\newhelp\chrerrormessage{La commande a deja ete definie.}%
\def\error!message{\errhelp{\the\chrhelpmessage}\errmessage{\the\chrerrormessage}} %
%
\def\!chrverif#1#2{\ifdefined#2\expandafter\error!message \fi #1#2}%
%
%Commandes utilis\'ees 
%
%
\def\!gobblethree#1#2#3{}%
\def\!gobble#1{}%
\ifdefined\@ifnextchar %LATEX
  \def\:{\let\ifnexttoken\@ifnextchar}\expandafter\:
\else 
  \ifdefined\doifnextcharelse %CONTEXT
    \def\:{\let\ifnexttoken\doifnextcharelse}\expandafter\:
  \else 
    \long\def\@ifnextchar#1#2#3{%
      \let\reserved@d=#1%
      \def\reserved@a{#2}%
      \def\reserved@b{#3}%
      \futurelet\@let@token\@ifnch}%
      \let\kernel@ifnextchar\@ifnextchar
      \def\@ifnch{%
        \ifx\@let@token\@sptoken
          \let\reserved@c\@xifnch
        \else
          \ifx\@let@token\reserved@d
            \let\reserved@c\reserved@a
          \else
            \let\reserved@c\reserved@b
          \fi
        \fi
    \reserved@c}%
\def\:{\let\@sptoken= }\: % this makes \@sptoken a space token
\def\:{\@xifnch}\expandafter\def\: {\futurelet\@let@token\@ifnch}%
\let\ifnexttoken\@ifnextchar
\fi\fi
%
\newif\if!chronearg \newif\if!chrtwoarg 
\!chrverif\def\!chrtraiteoneargument#1{\ifnexttoken[{\!chroneargtrue#1}{\!chroneargfalse#1[]}}%
%
\!chrverif\def\!chrtraitetwoargument#1{\let\todoafterarg#1%
\ifnexttoken[{\!chroneargtrue\savefirsttwoarg}{\!chroneargfalse\!chrtwoargfalse#1[][]}}%
\!chrverif\def\savefirsttwoarg[#1]{\ifnexttoken[{\!chrtwoargtrue \todoafterarg[#1]}{\!chrtwoargfalse \todoafterarg[#1][]}}%
%
\!chrverif\def\!chrtraitingargvirgule#1#2{\def\!tr@itintargvirgule{#2}\!chrtr@itingargvirgule#1,\end}%
\!chrverif\def\!chrtr@itingargvirgule#1,{%
\!chrdotraiteargvirgule#1,=\end,\ifnexttoken\end \!gobble \!chrtr@itingargvirgule}%
\!chrverif\def\!chrdotraiteargvirgule#1=#2,{%
\ifx \end#2\relax
\else \!chrdotr@iteargvirgule#1=#2,\expandafter\!gobblethree
\fi}%
\!chrverif\def\!chrdotr@iteargvirgule#1=#2,{%
\ifcsname \!tr@itintargvirgule#1\endcsname
 \expandafter\def\csname \!tr@itintargvirgule#1\endcsname{#2}%
\else \immediate\write16{chronosys : option #1 ligne \number\inputlineno\space non reconnue, impossible de lui affecter la valeur #2}%
\fi }%
%
%STARTCHRONOLOGY
%
\!chrverif\def\startchronology{\!chrtraiteoneargument\dostartchronology}%
%
%OPTIONS DE STARTCHRONOLOGY
%
\!chrverif\def\!chrdefaultstartyear{0}\!chrverif\def\!chrdefaultstopyear{\the\year}\!chrverif\def\!chrdefaultwidth{\the\hsize}%
\!chrverif\def\!chrdefaultheight{0.7pc}\!chrverif\def\!chrdefaultdates{true}\!chrverif\def\!chrdefaultarrow{true}% 
\!chrverif\def\!chrdefaultarrowwidth{0.1\!chrwidth}\!chrverif\def\!chrdefaultdateselevation{20pt}%
\!chrverif\def\!chrdefaultarrowheight{\!chrheight}\!chrverif\def\!chrdefaultcolor{black}\!chrverif\def\!chrdefaultarrowcolor{\!chr@color}%
\!chrverif\def\!chrdefaultdatesstyle{}\!chrverif\def\!chrdefaultstartdate{true}\!chrverif\def\!chrdefaultstopdate{true}% 
\!chrverif\def\!chrdefaultbox{false}\!chrverif\def\!chrdefaultalign{center}%
%
\!chr@verif\newdimen\!chrheight \!chr@verif\newif\if!chrdates \!chr@verif\newif\if!chrarrow \!chr@verif\newcount\!chrstartyear
\!chr@verif\newcount\!chrstopyear \!chr@verif\newdimen\!chrwidth \!chr@verif\newdimen\!chrarrowwidth \!chr@verif\newdimen\!chrarrowheight 
\!chr@verif\newbox\!chrflechebox 
\!chr@verif\newdimen\!chr!realwidth \!chr@verif\newdimen\!chr!unitperyear
\!chr@verif\newif\if!chrstartdate \!chr@verif\newif\if!chrstopdate \!chr@verif\newdimen\!chrdateselevation \!chr@verif\newif\if!chrbox
%
\!chrverif\def\!chr!periodeschwarzodergrau{\def\!chr!stringtest{black}%
\ifx\!chr@color\!chrstringtest
  \def\!chr!periodeschwarzodergr@u{gray}%
\else
  \def\!chr!periodeschwarzodergr@u{black}%
\fi}%
%
%
\!chr@verif\newdimen\!chrskipbefore
\!chr@verif\newdimen\!chrskipafter
%
\!chrverif\def\!chrdefaultoptions{startyear=\!chrdefaultstartyear, stopyear=\!chrdefaultstopyear,
startdate=\!chrdefaultstartdate, stopdate=\!chrdefaultstopdate,
height=\!chrdefaultheight, width=\!chrdefaultwidth, dates=\!chrdefaultdates, arrow=\!chrdefaultarrow,
arrowwidth=\!chrdefaultarrowwidth, arrowheight=\!chrdefaultarrowheight, color=\!chrdefaultcolor,
arrowcolor=\!chrdefaultarrowcolor, datesstyle=\!chrdefaultdatesstyle, dateselevation=\!chrdefaultdateselevation,
box=\!chrdefaultbox, align=\!chrdefaultalign}%
%
\!chrverif\def\!chr@startyear{}\!chrverif\def\!chr@startdate{}%
\!chrverif\def\!chr@stopyear{}\!chrverif\def\!chr@stopdate{}%
\!chrverif\def\!chr@height{}\!chrverif\def\!chr@width{}%
\!chrverif\def\!chr@dates{true}%
\!chrverif\def\!chr@arrow{}\!chrverif\def\!chr@arrowwidth{}\!chrverif\def\!chr@arrowheight{}% 
\!chrverif\def\!chr@color{}% 
\!chrverif\def\!chr@arrowcolor{}\!chrverif\def\!chr@datesstyle{}% 
\!chrverif\def\!chr@dateselevation{}%
\!chrverif\def\!chr@box{}\!chrverif\def\!chr@align{}%
%
%DOSTARTCHRONOLOGY
%
\!chrverif\def\dostartchronology[#1]{\begingroup\parindent\z@\par
\global\!chrskipafter\z@
\global\!chrskipbefore\z@
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter{\!chrdefaultoptions}{!chr@}%
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@}\fi 
\!chrheight\!chr@height   \!chrstartyear\!chr@startyear 
\!chrstopyear\!chr@stopyear    \!chrwidth\!chr@width %
\csname !chrdates\!chr@dates\endcsname \csname !chrarrow\!chr@arrow\endcsname 
\csname !chrstartdate\!chr@startdate\endcsname  \csname !chrbox\!chr@box\endcsname 
\csname !chrstopdate\!chr@stopdate\endcsname \!chrarrowwidth\!chr@arrowwidth 
\!chrarrowheight\!chr@arrowheight \!chrdateselevation\!chr@dateselevation%
\!chr!periodeschwarzodergrau%
\dostartchronologyfinal}%
%
\!chrverif\def\dostartchronologyfinal{%
\unless\if!chrarrow
  \!chrarrowwidth\z@\relax \!chrarrowheight\z@
\fi
\!chr!realwidth\dimexpr\!chrwidth-\!chrarrowwidth\relax
\ifdim\!chr!realwidth<0pt\relax
  \advance\!chrwidth\dimen@ 
  \advance\!chrarrowwidth-\!chr!realwidth 
  \!chr!realwidth\z@
\fi 
\dimen@\dimexpr\!chrheight-\!chrarrowheight\relax  
\dimen@ii\dimen@\relax
\ifdim\dimen@ii>0pt\relax
  \dimen@ii\z@
\fi
\dimen@i\dimexpr\!chrheight-\dimen@ii+\!chrdateselevation\relax
% % %AFFICHAGE DE LA FRISE
\setbox\!chrflechebox\hbox{%
  \if!chrdates
    \if!chrstartdate\raise\dimen@i\relax % %
      \hbox to\z@{\hss\!chr@datesstyle{\the\!chrstartyear}\hss}%
    \fi
  \fi%
%  \!chrstarttikzpicture\!chrfilldraw[color=\!chr@color](0,0)--(\the\!chr!realwidth,0)--(\the\!chr!realwidth,\the\!chrheight)--(0,\the\!chrheight)--cycle;
%  \if!chrbox
%    \!chrdraw[color=black](-0.4pt,-0.4pt)--(\the\!chr!realwidth+0.4pt,-0.4pt)--(\the\!chr!realwidth+0.4pt,\the\!chrheight+0.4pt)--(-0.4pt,\the\!chrheight)--cycle;
%  \fi %
%  \if!chrarrow
%    \ifx\!chr@color\!chr@arrowcolor
%    \else \!chrdraw[color=\!chr!periodeschwarzodergr@u](\the\!chr!realwidth,0)--(\the\!chr!realwidth,\the\!chrheight);
%    \fi
%  \fi
%  \!chrstoptikzpicture %
  \begingroup{%
  \!chrusecolor{\!chr@color}%
  \vrule width\!chr!realwidth height\!chrheight depth\z@\relax \kern-\!chr!realwidth\relax
  \if!chrbox
    \!chrusecolor{black}%
    \hbox to\z@{\vrule width\!chr!realwidth height0.4pt\relax\hss}%
    \raise\!chrheight\hbox to\z@{\vrule width\!chr!realwidth height0.4pt\relax\hss}%
    \vrule height\!chrheight depth\z@\relax\kern-0.4pt\relax
    \kern\!chr!realwidth \vrule height\!chrheight\relax\kern-0.4pt\relax
    \kern-\!chr!realwidth
  \fi
  %\if!chrarrow
  %\fi
  \kern\!chr!realwidth
  }%
  \endgroup
  \if!chrdates
    \if!chrstopdate
      \raise\dimen@i\hbox to\z@{\hss\!chr@datesstyle{\the\!chrstopyear}\hss}%
    \fi
  \fi%
%
  \if!chrarrow
    \raise0.5\dimen@\hbox{%
      \!chrstarttikzpicture
      \!chrfilldraw[color=\!chr@arrowcolor](0,0.5*\the\!chrarrowheight-0.4pt)--(\the\!chrarrowwidth,0)--(0,-0.5*\the\!chrarrowheight)--cycle;
      \if!chrbox
        \!chrdraw[color=black](-0.4pt,0.5*\the\!chrarrowheight+0.4pt)--(\the\!chrarrowwidth+0.4pt,0)--(-0.4pt,-0.5*\the\!chrarrowheight-0.4pt)--cycle;
      \fi
      \!chrstoptikzpicture
      \edef\@@string@a{\!chr@color}%
      \edef\@@string@b{\!chr@arrowcolor}%
      \ifx\@@string@a\@@string@b
      \else
        {\!chrusecolor{\!chr!periodeschwarzodergr@u}%
        \kern-\!chrarrowwidth\kern-0.2pt\relax \hbox to\z@{\vrule height\dimexpr(\!chrarrowheight-\!chrheight)/2 + \!chrheight\relax depth\dimexpr(\!chrheight-\!chrarrowheight)/2\relax\hss}% 
        \kern\!chrarrowwidth\kern-0.2pt\relax}%
      \fi
    }%
  \fi}%
  \count@\numexpr\!chrstopyear-\!chrstartyear\relax
  \ifnum\count@<0\relax
    \immediate\write16{Erreur avec les dates donn\'ees}%
  \fi 
  \!chr!unitperyear\dimexpr\!chr!realwidth/\count@\relax}%
%
%
\!chrverif\def\setupchronology#1{\!chrtraitingargvirgule{#1}{!chrdefault}}%
%
%PERIODES
%
\!chr@verif\newcount\!chr!periodecolornum\!chr@verif\newcount\!chr!starttingtraitement \!chr@verif\newdimen\!chr!dimentraitement
\!chr@verif\newdimen\!chrperiodtextdepth \!chrverif\def\!chrperiodedefaulttextdepth{15pt}% 
\!chr@verif\newif\if!chrperioddates  \!chr@verif\newif\if!chrperiodbox
\!chr@verif\newif\if!chrperiodstartdate \!chr@verif\newif\if!chrperiodstopdate \!chrverif\def\!chrperiodedefaultstartdate{true}
\!chr@verif\newif\if!chrperiodifcolorbox 
\!chr@verif\newdimen\!chrperioddateselevation 
\!chr@verif\newdimen\!chrperiodeventtextwidth 
\!chr@verif\newdimen\!chrperiodbottomdepth \!chr@verif\newdimen\!chrperiodtopheight
%
%alternance des couleurs
\!chr@verif\newcount\!chrperiodecoloralternancetotalnum
\!chrverif\def\!chrperiodedefaultcolor{\chronoperiodcolor}%
\!chrverif\def\!chrperiodedefa@@ultcolor{\chronoperiodcolor}%
\!chrverif\def\!chrperiodedef@ultcolor{\!chrperiodedefaultcolor}%
\!chrverif\def\chronoperiodcolor{\ifcase\!chr!periodecolornum blue\or red\or cyan\or purple\or yellow\fi}%
\!chrperiodecoloralternancetotalnum5%
\!chrverif\def\!chr!periodecolor{\edef\!chrperiodedef@ultcolor{\!chrperiodedefaultcolor}%
  \ifx\!chrperiodedefaultcolor\!chrperiodedefa@@ultcolor
    \ifx\!chrperiodedef@ultcolor\!chr@color
      \!chr!periodecoloradvance\!chr!periodecolor 
    \fi
  \fi}%
\!chrverif\def\!chr!periodecoloradvance{\global\advance\!chr!periodecolornum\@ne\relax
\ifnum\!chr!periodecolornum=\!chrperiodecoloralternancetotalnum\relax\global\!chr!periodecolornum\z@\fi}%
%
\!chrverif\def\restartchronoperiodecolor{\!chrtraiteoneargument\dorestartchronoperiodecolor}%
\!chrverif\def\dorestartchronoperiodecolor[#1]{%
\if!chronearg 
  \def\@@string@a{#1}%
  \!chr!periodecolornum\z@ %
  \dorestartchronoperiodecolor@ux
\else
  \!chr!periodecolornum\z@
\fi}%
\!chrverif\def\dorestartchronoperiodecolor@ux{\edef\@@string@b{\chronoperiodcolor}%
\ifnum\!chr!periodecolornum<\!chrperiodecoloralternancetotalnum
  \unless\ifx\@@string@a\@@string@b
    \global\advance\!chr!periodecolornum\@ne 
    \dorestartchronoperiodecolor@ux
  \fi
\else\global\!chr!periodecolornum\z@\fi}%
%
\!chrverif\def\chronoperiodecoloralternation#1{%
\def\@@string@s{\ifcase\!chr!periodecolornum}%
\!chrperiodecoloralternancetotalnum\z@\!chr!chronoperiodecoloralternance#1,\end \let\chronoperiodcolor\@@string@s
\!chr!periodecolornum\z@}%
%
\!chrverif\def\!chr!chronoperiodecoloralternance#1,{\advance\!chrperiodecoloralternancetotalnum\@ne
\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s#1}%
\ifnexttoken\end {\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s\fi}\!gobble}%
{\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s\or}\!chr!chronoperiodecoloralternance}}%
%
%
\!chrverif\def\!chr@periodtextdepth{}\!chrverif\def\!chr@perioddates{}%
\!chrverif\def\!chr@periodcolor{}\!chrverif\def\!chr@perioddatesstyle{}%
\!chrverif\def\!chr@periodstartdate{}\!chrverif\def\!chr@periodstopdate{}%
\!chrverif\def\!chr@periodtextstyle{}%
\!chrverif\def\!chr@perioddateselevation{}%
\!chrverif\def\!chr@periodifcolorbox{}\!chrverif\def\!chr@periodcolorbox{}%
\!chrverif\def\!chr@periodbottomdepth{}\!chrverif\def\!chr@periodtopheight{}%
\!chrverif\def\!chr@periodbox{}\!chrverif\def\!chr@periodtextwidth{}%
%
\!chrverif\def\!chreventdefaulttesttextwidth{\relax}%
%
%DOCHRONOPERIODE
%
%
\!chrverif\def\dochronoperiode[#1]#2#3#4{%
\!chr!periodecolor %alternance automqatique des couleurs
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@period}\fi
% % %
\!chrperiodtextdepth\!chr@periodtextdepth \!chrperiodtopheight\!chr@periodtopheight
\!chrperiodbottomdepth\!chr@periodbottomdepth
\csname !chrperioddates\!chr@perioddates\endcsname \csname !chrperiodstartdate\!chr@periodstartdate\endcsname 
\csname !chrperiodstopdate\!chr@periodstopdate\endcsname \csname !chrperiodifcolorbox\!chr@periodifcolorbox\endcsname
\csname !chrperiodbox\!chr@periodbox\endcsname
\ifx\!chr@periodtextwidth\!chreventdefaulttesttextwidth
	\!chrperiodeventtextwidth=-1pt%
\else
	\!chrperiodeventtextwidth=\!chr@periodtextwidth%
\fi
\!chrperioddateselevation\!chr@perioddateselevation 
\advance\!chrperioddateselevation 1.25\!chrheight\relax
% % %On s'assure que les dates sont biebn dans l'intervalle
\ifnum#2>\numexpr\!chrstartyear-1\relax
\ifnum#2<\numexpr\!chrstopyear+1\relax
\ifnum#3<\numexpr\!chrstopyear+1\relax 
\ifnum#3>\numexpr\!chrstartyear-1\relax
\count@\numexpr#3-#2\relax
% % %Et que la seconde est post\'erieure \`a la pr\'emi\`ere
\ifnum\count@>\z@\relax
% %
\!chr!starttingtraitement\numexpr#2-\!chrstartyear\relax\dimen@\dimexpr\count@\!chr!unitperyear\relax
\!chr!dimentraitement\dimexpr\!chr!starttingtraitement\!chr!unitperyear\relax
% %AFFICHAGE
\dimen@i\wd\!chrflechebox
\setbox\!chrflechebox\hbox{%
  \unhbox\!chrflechebox\kern-\dimen@i\kern\!chr!dimentraitement
  \lower\dimexpr\!chrperiodtextdepth-\!chrperiodbottomdepth\relax\hbox to\z@{%
    \ifdim\!chrperiodeventtextwidth < \z@ \hbox to\dimen@{%
      	\hss \if!chrperiodifcolorbox\expandafter\!chrperiodcolorbox\fi{\!chr@periodtextstyle{#4}}\hss
    	}%
    \else
       \setbox\z@\hbox to\dimen@{\hss\vbox{%
       \hsize\!chrperiodeventtextwidth {\!chr@periodtextstyle{#4}}
       }\hss}%
       \dimen@i\wd\z@
       \dimen@ii\dimexpr\ht\z@+\dp\z@\relax
       \lower\dimexpr\dimen@ii-10pt\relax\hbox to\dimen@{%
          \hss\setbox\z@\hbox{%
           \vbox{%
            \hsize\!chrperiodeventtextwidth\relax\!chr@periodtextstyle{#4}%
            \vskip1pt
           }%
          }%
          \dimen@i\dimexpr\wd\z@+4pt\relax
          \dimen@ii\dimexpr\ht\z@+\dp\z@+2pt\relax
          \setbox\z@\hbox to\z@{%
          \hss\begingroup{\!chrusecolor{\!chr@periodcolorbox}\vrule height\dimen@ii width\dimen@i depth2pt}\endgroup\kern-\dimen@i\kern2pt\relax%
                     \box\z@\hss
          }%
          \box\z@\hss
       }%
    \fi
    \hss
  }%
  \if!chrperioddates
    \if!chrperiodstartdate
      \raise\dimexpr\!chrperioddateselevation +(\!chrperiodtopheight-\!chrheight)\relax 
      \hbox to\z@{%
        \hss\!chr@perioddatesstyle{#2}\hss
      }%
    \fi
  \fi 
  \raise\!chrperiodbottomdepth \hbox{%
    \begingroup {\!chrusecolor{\!chr@periodcolor}%
       \dimen@i\dimexpr\!chrperiodtopheight-\!chrperiodbottomdepth\relax%
       \vrule width\dimen@ height\dimen@i depth\z@\kern-\dimen@%
%       \!chrusecolor{black}%
%       \raise\dimen@i\hbox to\z@{\vrule height0.1pt depth0.3pt width\dimen@\hss}%
%       \hbox to\z@{\vrule height0.1pt depth0.3pt width\dimen@\hss}%
    }\endgroup%%
    \begingroup{%
    \dimen@i\dimexpr\!chrperiodtopheight-\!chrperiodbottomdepth\relax%
    \!chrusecolor{\!chr!periodeschwarzodergr@u}%
    \kern-0.2pt\relax\vrule height\dimen@i width0.4pt\relax  \kern-0.2pt\relax%
    \kern\dimen@\relax
    \kern-0.2pt\relax\vrule height\dimen@i width0.4pt\relax  \kern-0.2pt\relax
    \kern-\dimen@\relax
    }%
    \endgroup
    \begingroup{%
    \!chrusecolor{black}
    \if!chrbox
      \lower 0.2pt\hbox to\z@{\vrule width\dimen@\hss}%
    \fi
    \if!chrperiodbox
      \raise \!chrperiodbottomdepth \hbox to\z@{\vrule width\dimen@\hss}%
      \raise \!chrperiodtopheight \hbox to\z@{\vrule width\dimen@\hss}%
    \fi
    }%
    \endgroup
    \kern\dimen@\relax
  }%
  \if!chrperioddates
    \if!chrperiodstopdate
      \raise\dimexpr\!chrperioddateselevation+(\!chrperiodtopheight-\!chrheight)\relax
      \hbox to\z@{%
        \hss \!chr@perioddatesstyle{#3}\hss
      }%
    \fi
  \fi
}%
\!chr!periodecoloradvance
\fi\fi\fi\fi\fi}%
%
%
\!chrverif\def\setupchronoperiode{\def\@@string@a{periode}\!chrtraiteoneargument\dosetupchronoeventandperiode}%
%
%EVENTS
%
%
\!chr@verif\newif\if!chreventspecifiedday\!chr@verif\newif\if!chreventspecifiedmonth \!chr@verif\newif\if!chreventbarre
\!chr@verif\newif\if!chreventdate  \!chr@verif\newif\if!chreventmark
\!chr@verif\newif\if!chreventifcolorbox \!chr@verif\newif\if!chreventconversionmonth 
\!chr@verif\newdimen\!chreventmarkdepth \!chr@verif\newif\if!chreventyear \!chr@verif\newdimen\!chreventiconheight
 \!chrverif\def\!chreventdefaultbarre{true}%
\!chrverif\def\!chreventdefaulticon{}%
\!chrverif\def\!chreventdefaultmarkdepth{10pt}%
\!chrverif\def\!chreventdefaulttextstyle{}%
%
%
%
\!chrverif\def\!chreventevalspecification#1{\count@\z@\relax\!chreventev@lspecification#1/\end}%
\!chrverif\def\!chreventev@lspecification#1/{\advance\count@\@ne\relax\expandafter\def\csname
!chreventspecifiedargument\number\count@\endcsname{#1}\ifnexttoken\end \!gobble \!chreventev@lspecification}%
%
\!chrverif\def\chron@selectmonth#1{\ifcase#1\or janvier\or f\'evrier\or mars\or avril\or mai\or juin\or juillet\or ao\^ut\or septembre\or octobre\or novembre\or d\'ecembre\fi}%
%
\!chrverif\def\!chr@eventbarre{}\!chrverif\def\!chr@eventicon{}\!chrverif\def\!chr@eventmarkdepth{}%
\!chrverif\def\!chr@eventtextstyle{}\!chrverif\def\!chr@eventmark{}%
\!chrverif\def\!chr@eventdate{}\!chrverif\def\!chr@eventdatesseparation{}%
\!chrverif\def\!chr@eventconversionmonth{}\!chrverif\def\!chr@eventdatestyle{}%
\!chrverif\def\!chr@eventdatesstyle{}\!chrverif\def\!chr@eventyear{}\!chrverif\def\!chr@eventiconheight{}%
\!chrverif\def\!chr@eventifcolorbox{}\!chrverif\def\!chr@eventcolorbox{}%.
\!chrverif\def\!chr@eventtextwidth{}%
% 
\!chr@verif\newif\if!chreventlocationup
%
%
%DOCHRONOEVENT
%
%
\!chrverif\def\dochronoevent[#1]#2#3{%
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@event}\fi
% % %
\csname !chreventbarre\!chr@eventbarre\endcsname 
\csname !chreventmark\!chr@eventmark\endcsname 
\csname !chreventdate\!chr@eventdate\endcsname
\csname !chreventconversionmonth\!chr@eventconversionmonth\endcsname 
\csname !chreventyear\!chr@eventyear\endcsname
\csname !chreventifcolorbox\!chr@eventifcolorbox\endcsname
\!chreventmarkdepth\!chr@eventmarkdepth 
\!chreventiconheight\!chr@eventiconheight
\ifx\!chr@eventtextwidth\!chreventdefaulttesttextwidth 
   \!chrperiodeventtextwidth=-1pt%
\else \!chrperiodeventtextwidth\!chr@eventtextwidth
\fi
\ifdim\!chreventmarkdepth<\z@\relax
  \!chreventlocationuptrue
\else
  \!chreventlocationupfalse
\fi
% % % Evaluation de la precision de la date de l'evenement
\!chreventevalspecification{#2}%
\ifnum\count@<4\relax
  \ifcase\count@
    \or \!chreventspecifieddayfalse\!chreventspecifiedmonthfalse 
        \edef\!chreventyear{\csname !chreventspecifiedargument1\endcsname}%
    \or \!chreventspecifieddayfalse\!chreventspecifiedmonthtrue
        \edef\!chreventyear{\csname !chreventspecifiedargument2\endcsname}%
        \edef\!chreventmonth{\csname !chreventspecifiedargument1\endcsname}%
    \or \!chreventspecifieddaytrue\!chreventspecifiedmonthtrue
        \edef\!chreventyear{\csname !chreventspecifiedargument3\endcsname}%
        \edef\!chreventmonth{\csname !chreventspecifiedargument2\endcsname}%
        \edef\!chreventday{\csname !chreventspecifiedargument1\endcsname}%
  \fi %
% %On s'assure que les dates sont bien comprises dans les bornes
\ifnum\!chreventyear>\numexpr\!chrstartyear-1\relax
\ifnum\!chreventyear<\numexpr\!chrstopyear+1\relax
      \if!chreventspecifiedmonth
        \if!chreventspecifiedday 
          \count@\numexpr\!chreventday+\!chreventmonth*30\relax
        \else %
          \count@\numexpr\!chreventmonth*30\relax
        \fi
      \else \count@\z@
      \fi %
      \!chr!dimentraitement\dimexpr(\!chr!unitperyear)/365*\count@\relax%
     \count@\numexpr\!chreventyear-\!chrstartyear\relax 
     \advance\!chr!dimentraitement\dimexpr\count@\!chr!unitperyear\relax
% % % Affichage
     \dimen@i\wd\!chrflechebox
     \setbox\!chrflechebox\hbox{%
       \unhbox\!chrflechebox\kern-\dimen@i\kern\!chr!dimentraitement
       \if!chreventbarre
        \begingroup{%
        \!chrusecolor{black}%
        \kern-0.4pt\relax\vrule width0.4pt height\!chrheight depth\z@\relax
        }%
        \endgroup
       \fi
       \kern-0.4pt\raise\!chreventiconheight \hbox to\z@{\hss\!chr@eventicon\hss}%
       \lower\dimexpr\!chreventmarkdepth+2pt\relax
       \hbox to\z@{%
         \vbox to\z@{%
           \if!chreventlocationup\relax\vss\fi
           \if!chreventdate\hbox to\z@{%
             \hss \if!chreventifcolorbox \expandafter\!chreventcolorbox\fi
             {\!chr@eventdatestyle{%
               \if!chreventspecifiedday %
                 {\!chr@eventdatesstyle{\!chreventday}}\!chr@eventdatesseparation
               \fi
             {\!chr@eventdatesstyle{%
               \if!chreventspecifiedmonth 
                 \if!chreventconversionmonth\expandafter \chron@selectmonth
                 \fi 
                 \!chreventmonth
               \fi
               }%
             }%
             \if!chreventspecifiedmonth\if!chreventyear \!chr@eventdatesseparation\fi\fi 
             \if!chreventyear{\!chr@eventdatesstyle{\!chreventyear}}\fi%
             }}%
             \hss
           }%
           \fi
           \ifdim\!chrperiodeventtextwidth > \z@ 
             \hbox to\z@{%
               \hss\setbox\z@\hbox{%
                 \vbox{%
                   \hsize\!chrperiodeventtextwidth\relax\!chr@eventtextstyle{#3}%
                   \vskip1pt\relax
                 }%
               }%
               \dimen@i\dimexpr\wd\z@+4pt\relax
               \dimen@ii\dimexpr\ht\z@+\dp\z@+2pt\relax
               \setbox\z@\hbox to\z@{%
                 \hss\begingroup{\!chrusecolor{\!chr@eventcolorbox}\vrule height\dimen@ii width\dimen@i depth2pt\relax}\endgroup \kern-\dimen@i\kern2pt\relax%
                 \box\z@\hss
               }%
               \box\z@
             }%
           \else 
             \hbox to\z@{%
               \hss\if!chreventifcolorbox\expandafter\!chreventcolorbox\fi{%
               \!chr@eventtextstyle{#3}}\hss
             }%
           \fi 
           \unless\if!chreventlocationup\relax\vss\fi
         }%
       }%
       \if!chreventmark
         \if!chreventlocationup\relax
         %\!chrstarttikzpicture \!chrdraw(0,0)--(0,\the\!chreventmarkdepth+5pt);\!chrstoptikzpicture
           \vrule height\dimexpr-\!chreventmarkdepth-5pt\relax depth\z@ \kern-0.4pt\relax
         \else \vrule height\z@ depth\!chreventmarkdepth
         \fi
         \kern-0.4pt\relax
       \fi  
       \setbox0\vbox{%
         \if!chreventdate
           \hbox{#2}%
         \fi
         \hbox{%
          \ifdim\!chrperiodeventtextwidth > \z@ 
            \vbox {%
             \hsize\!chrperiodeventtextwidth #3%
            }%
          \else #3%
          \fi 
         }%
       }%
      \begingroup\dimen@\dimexpr\dp0+\ht0+2pt\relax
      \dimen@i\dimexpr\dimen@-\!chreventmarkdepth\relax
      \if!chreventlocationup
        \ifdim \dimen@i >\!chrskipbefore \global\!chrskipbefore\dimen@i \fi
      \else
        \ifdim \dimen@ >\!chrskipafter \global\!chrskipafter\dimen@ \fi
      \fi
      \endgroup
    }%
\fi\fi\fi}%
%
%
%
%
%
%
%
\!chrverif\def\setupchronoevent{\def\@@string@a{event}\!chrtraiteoneargument\dosetupchronoeventandperiode}%
\!chrverif\def\dosetupchronoeventandperiode[#1]#2{\if!chronearg
\def\@@string@a{#1}\fi \!chr@parcoursoptions#2,\end}%
%
%STOPCHRONOLOGY
%
%
\!chr@verif\newdimen\!chrstopwidth
\!chrverif\def\!chrstopcenteralign{\!chrstopwidth\dimexpr(\hsize-\!chrwidth)/2\relax}%
\!chrverif\def\!chrstopleftalign{\!chrstopwidth\z@}%
\!chrverif\def\!chrstoprightalign{\!chrstopwidth\dimexpr\hsize-\!chrwidth\relax}%
%
\!chrverif\def\stopchronology{\goodbreak
\ifcsname !chrstop\!chr@align align\endcsname
  \csname !chrstop\!chr@align align\endcsname
\else\!chrstopwidth\z@
\fi 
\vskip\!chrskipbefore
\moveright\!chrstopwidth\box\!chrflechebox
\vskip\!chrskipafter
\endgroup\bigskip}%
%
\!chr@verif\newif\if!chrverifdefines
\!chrverif\def\!chrverifdefines{%
 \ifcsname chrono\@@string@a\endcsname
   \!chrverifdefinesfalse \immediate\write16{Attention : macro \expandafter\noexpand\csname chrono\@@string@a\endcsname deja definie.}%
   \expandafter\!gobble 
 \else
   \!chrverifdefinestrue
   \expandafter\!chrverifdefines@ux
 \fi}%
\!chrverif\def\!chrverifdefines@ux{\expandafter\def\csname chrono\@@string@a\endcsname}%
%
%
%DEFINECHRONOEVENT
%
%
\!chrverif\def\definechronoevent#1{%
\def\@@string@a{#1}%
\!chrverifdefines{%
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter\expandafter\expandafter{\csname !chr#1defaultoptions\endcsname}{!chr@event}%
\!chrtraiteoneargument\dochronoevent}%
\if!chrverifdefines
  \expandafter\def\csname !chr#1defaultoptions\endcsname{barre=true, icon=\relax,%
  markdepth=10pt, textstyle=\relax, mark=true,%
  date=true, datesseparation=\space, conversionmonth=true,%
  datestyle=\relax, datesstyle=\relax, year=true,%
  iconheight=0.5\!chrheight, ifcolorbox=true, colorbox=white,%
  textwidth=\relax}%
\fi
\ifnexttoken[{\!chr@defineorsetupoptions}{}}%
%
%
%DEFINECHRONOPERIODE
%
%
\!chrverif\def\definechronoperiode#1{%
\def\@@string@a{#1}%
\!chrverifdefines{%
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter\expandafter\expandafter{\csname !chr#1defaultoptions\endcsname}{!chr@period}%
\!chrtraiteoneargument\dochronoperiode}%
\if!chrverifdefines
  \expandafter\def\csname !chr#1defaultoptions\endcsname{textdepth=15pt, dates=true,%
  color=\!chrperiodedef@ultcolor, datesstyle=\relax,%
  startdate=true, stopdate=true, textstyle=\relax,%
  dateselevation=0pt, ifcolorbox=true,%
  colorbox=white, bottomdepth=0pt, topheight=\!chrheight, box=false,%
  textwidth=\relax}%
\fi
\ifnexttoken[{\!chr@defineorsetupoptions}{}}%
%
%pour modifier les valeurs par d\'efaut
%
\!chrverif\def\!chr@defineorsetupoptions[#1]{%
\!chr@parcoursoptions#1,\end
}%
%
\!chrverif\def\!chr@parcoursoptions#1,{\!chr@replaceoptions#1,=\end,\ifnexttoken\end \!gobble \!chr@parcoursoptions}%
\!chrverif\def\!chr@replaceoptions#1=#2,{%
\ifx#2\end\relax
\else
  \def\@@string@f{}%
  \def\@@string@c{#1}\def\@@string@d{#2}%
  \expandafter\let\expandafter\@@string@@b\csname !chr\@@string@a defaultoptions\endcsname
  \expandafter\!chr@replaceoptionsaux\@@string@@b,\end%
  \expandafter\let\csname !chr\@@string@a defaultoptions\endcsname\@@string@f
  \expandafter\!gobblethree
\fi}%
%
\!chrverif\def\!chr@replaceoptionsaux#1,{\!chr@replaceoptions@ux#1,=\end,\ifnexttoken\end\!gobble\!chr@replaceoptionsaux}%
\!chrverif\def\!chr@replaceoptions@ux#1=#2,{%
\ifx#2\end\relax
\else
  \def\@@string@e{#1}% 
  \ifx\@@string@c\@@string@e
    \expandafter\def\expandafter\@@string@f\expandafter{\@@string@f , #1=}%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@@string@f\expandafter\expandafter\expandafter{\expandafter\@@string@f\@@string@d}%
  \else 
    \expandafter\def\expandafter\@@string@f\expandafter{\@@string@f , #1=#2}%
  \fi
  \expandafter\!gobblethree
\fi
}%
%
%
\!chr@verif\newcount\!chrgraduationcount
\!chr@verif\newcount\!chrgraduationcount@ux
\newif\if!chrgradu@tionevent \!chrgradu@tioneventtrue
\!chrverif\def\chronograduation{\!chrtraitetwoargument\dochronograduation}%
\!chrverif\def\dochronograduation[#1][#2]#3{%
\if!chrtwoarg
  \def\@@string@a{#2}%
  \def\@@string@b{#1}\def\@@string@c{event}%
  \def\@@string@d{periode}%
  \ifx\@@string@b\@@string@c 
    \!chrgradu@tioneventtrue 
  \else
    \ifx\@@string@b\@@string@d 
      \!chrgradu@tioneventfalse
    \else 
    	\def\@@string@e{}\unless\ifx\@@string@b\@@string@e\immediate\write16{chronosys : style #1 non défini ligne \number\inputlineno}\fi
    \fi
  \fi 
\else \def\@@string@a{#1}%
\fi
\!chrgraduationcount\!chrstartyear
\if!chrgradu@tionevent
  \loop
    \advance\!chrgraduationcount#3%
    \ifnum\!chrgraduationcount<\!chrstopyear 
      \expandafter\chrono!!eventgradu@tion
      \expandafter[\@@string@a]{\number\!chrgraduationcount}{}%
  \repeat
\else 
  \def\@@string@e{startdate=true,}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@@string@e\expandafter\expandafter\expandafter{\expandafter\@@string@e\@@string@a}%
  \expandafter\chrono!!periodegradu@tion\expandafter[\@@string@e]{\number\!chrgraduationcount}{#3}{}%
  \restartchronoperiodecolor
  \loop 
    \advance\!chrgraduationcount#3%
    \ifnum\!chrgraduationcount<\!chrstopyear
       \!chrgraduationcount@ux\numexpr\!chrgraduationcount-#3\relax \expandafter\chrono!!periodegradu@tion\expandafter[\@@string@a]{\number\!chrgraduationcount@ux}{\number\!chrgraduationcount}{}%
  \repeat
\fi}%
%
\!chrverif\def\setupchronograduation{\!chrtraiteoneargument\dosetupchronograduation}%
\!chrverif\def\dosetupchronograduation[#1]{%
\if!chronearg
  \def\@@string@b{#1}\def\@@string@c{event}\def\@@string@d{periode}%
  \ifx\@@string@b\@@string@c 
    \!chrgradu@tioneventtrue 
  \else
    \ifx\@@string@b\@@string@d 
      \!chrgradu@tioneventfalse
    \fi
  \fi 
\fi
\if!chrgradu@tionevent 
  \def\@@string@a{[!!eventgradu@tion]}%
\else \def\@@string@a{[!!periodegradu@tion]}%
\fi
\expandafter\setupchronoevent\@@string@a}%
%
\definechronoevent{event}%
\definechronoevent{!!eventgradu@tion}[markdepth=5pt,barre=false, ifcolorbox=false]%
\definechronoperiode{periode}%
\definechronoperiode{!!periodegradu@tion}[dateselevation=-10pt,%
startdate=false, ifcolorbox=false]%
%
\endinput
%
%

==> fullspecifications.tex <==

%\afterpage{%
%    \clearpage% Flush earlier floats (otherwise order might not be correct)
%    \thispagestyle{empty}% empty page style (?)
%    \begin{landscape}% Landscape page
 %       \centering % Center table
\begin{table*}[!t]
\scriptsize
\caption{Technical specifications of various LPWA technologies}
\label{tab:specifications}
\vspace{-2mm}
\centering
\hspace*{-6mm}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
\begin{tabulary}{1\textwidth} {|J|J|J|J|J|J|J|J|J|J|J|J| }\hline
%& \multicolumn{10}{c|}{\textbf{updates sent in a given epoch}}\\
%\cline{2-17}
& \sigfox  
& \lorawan 
& \weightless 
& \ingenu 
& \telensa % Telensa 
& \qowisio 
& \dash  
& IEEE 802.15.4k 
& IEEE 802.15.4g
& ETSI LTN 
& 3GPP \nbiot 
\\\hline
\textbf{Modulation}  %<---------------
& UNB DBPSK\ul, GFSK\dl %\sigfox  
& CSS %\lorawan 
& UNB(N) %\weightless 
& \rpma-DSSS\ul, CDMA\dl%\ingenu 
& UNB FSK %\telensa
& UNB %\qowisio
& GFSK %DASH-7   
& DSSS, FSK%IEEE 802.15.4k 
& MR-(FSK,OFDMA,OQPSK)%IEEE 802.15.4g
& UNB (BPSK\ul\usman{No Listen before talk (LBT) or adaptive frequency agility (AFA)}, GFSK\dl) or OSSS%ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Band} %<---------------
& \subghz \ism:EU (868MHz), US(902MHz) %\sigfox  
& \subghz \ism:EU (433MHz 868MHz), US (915MHz), Asia (430MHz) %\lorawan 
& \subghz \ism or TV whitespaces %\weightless 
& \ism 2.4GHz %\ingenu 
& \subghz \ism:EU (868MHz), US (915MHz), Asia (430MHz) %\telensa
& %\qowisio
& \subghz 433MHz, 868MHz, 915MHz %DASH-7   
& \ism \subghz \& 2.4GHz%IEEE 802.15.4k 
& \ism \subghz \& 2.4GHz %IEEE 802.15.4g
& \subghz \ism %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Forward error correction} %<---------------
& \xmark %\sigfox  
& \cmark %\lorawan 
& %\weightless 
& \cmark %\ingenu 
& %\telensa
& %\qowisio
& \cmark %DASH-7   
& \cmark %IEEE 802.15.4k 
& \cmark %IEEE 802.15.4g
& \xmark (error detection only) %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{PHY Multiple Access}  %<--------------- 
& 360 channels%\sigfox  
& Multiple SFs, Channels: EU(10), US(64+8\ul,8\dl )   %\lorawan 
& Multiple 200Hz channels (N) %\weightless 
& 40 1MHz channels, up to 1200 signals per channel  %\ingenu 
& %\telensa
& %\qowisio
& 3 types of channels (number depends on band \&region)%DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& \nd %ETSI LTN 
& %NB-IoT 

\\\hline
\textbf{MAC}  %<--------------- 
& Unslotted \aloha%\sigfox  
& Unslotted \aloha %\lorawan 
& %\weightless 
& CDMA-like %\ingenu
& %\telensa 
& %\qowisio
& %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& \nd %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Data rate} %<---------------
& 100 bps\ul, 600 bps\dl %\sigfox  
& 0.3-37.5 kbps (\lora), 50 kbps (FSK) %\lorawan 
& %\weightless 
& 78kbps \ul, 19.5 kbps\dl~\cite{comparisontable} \usman{156 kbps per sector with 8 channels but 10 kbps http://www.slideshare.net/MaartenWeyn1/overview-of-low-power-wide-area-networks} %\ingenu
& 62.5 bps\ul, 500 bps\dl  %\telensa 
& %\qowisio
& 9.6, 55, 167 kbps %DASH-7   
& 1.5bps-128kbps %IEEE 802.15.4k 
& 4.8kbps-800kbps%IEEE 802.15.4g
& %ETSI LTN 
& %NB-IoT 
\\\hline

\textbf{Adaptive Data Rate}  %<---------------
& \xmark (end device does not join a specific base station)%\sigfox  
& \cmark %\lorawan 
& %\weightless 
& \cmark %\ingenu 
& \xmark %\telensa
& \xmark %\qowisio
& \xmark %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& %ETSI LTN 
& %NB-IoT 
\\\hline


\textbf{Payload length}  %<---------------
& 12B\ul, 8B\dl %\sigfox  
& up to 250B (depends on SF \& region)%\lorawan 
& %\weightless 
& 10KB %\ingenu
& %\telensa 
& %\qowisio
& 256B %DASH-7   
& 2047B%IEEE 802.15.4k 
& 2047B%IEEE 802.15.4g
& 255B %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Over the air updates}  %<---------------
& \xmark %\sigfox  
& under development %\lorawan 
& %\weightless 
& %\ingenu
& \xmark %\telensa 
& %\qowisio
& possible %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& \nd %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Authentication \& encryption}  %<---------------
& Encryption not supported %\sigfox  
& AES 128b  %\lorawan 
& %\weightless 
& 16B hash, AES 256b %\ingenu 
& %\telensa
& %\qowisio
& AES 128b%DASH-7   
& AES 128b %IEEE 802.15.4k 
& AES 128b%IEEE 802.15.4g
& \cmark %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Handover}  %<---------------
& end devices do not join a single base station %\sigfox  
& end devices do not join a single base station %\lorawan 
& %\weightless 
& \cmark %\ingenu 
& %\telensa
& %\qowisio
& \cmark%DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& \cmark %ETSI LTN 
& %NB-IoT 
\\\hline
%\textbf{Roaming support}  %<---------------
%& %\sigfox  
%& %\lorawan 
%& %\weightless 
%& %\ingenu
%& %\telensa 
%& %\qowisio
%& %DASH-7   
%& %IEEE 802.15.4k 
%& %IEEE 802.15.4g
%& \cmark %ETSI LTN 
%& %NB-IoT 
%\\\hline
\textbf{SLA support}  %<---------------
& \xmark %\sigfox  
& \xmark %\lorawan 
& %\weightless 
& \xmark %\ingenu
& \xmark %\telensa 
& \xmark %\qowisio
& \xmark %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Link symmetry}  %<---------------
& \xmark %\sigfox  
& \cmark %\lorawan 
& %\weightless 
&  \xmark %\ingenu 
& \xmark %\telensa
& %\qowisio
& %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{Localization}  %<---------------
& \xmark %\sigfox  
& \cmark %\lorawan 
& \xmark%\weightless 
& \xmark%\ingenu 
& \xmark%\telensa
& \xmark%\qowisio
& \xmark%DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& %ETSI LTN 
& %NB-IoT 
\\\hline
\textbf{No. of devices}  %<---------------
& %\sigfox  
& %\lorawan 
& %\weightless 
& 16k\usman{from telefonica}%\ingenu 
& 5k %\telensa
& %\qowisio
& %DASH-7   
& %IEEE 802.15.4k 
& %IEEE 802.15.4g
& \cmark %ETSI LTN 
& %NB-IoT 
\\\hline
%\end{tabular}
\end{tabulary}
\vspace*{-6mm}
\end{table*}
%       \captionof{table}{Table caption}% Add 'table' caption
%    \end{landscape}
%    \clearpage% Flush page
%}


